Dialogue Disentanglement in Software Engineering: How Far are We?

Despite the valuable information contained in software chat messages, disentangling them into distinct conversations is an essential prerequisite for any in-depth analyses that utilize this information. To provide a better understanding of the current state-of-the-art, we evaluate five popular dialog disentanglement approaches on software-related chat. We find that existing approaches do not perform well on disentangling software-related dialogs that discuss technical and complex topics. Further investigation on how well the existing disentanglement measures reflect human satisfaction shows that existing measures cannot correctly indicate human satisfaction on disentanglement results. Therefore, in this paper, we introduce and evaluate a novel measure, named DLD. Using results of human satisfaction, we further summarize four most frequently appeared bad disentanglement cases on software-related chat to insight future improvements. These cases include (i) ignoring interaction patterns; (ii) ignoring contextual information; (iii) mixing up topics; and (iv) ignoring user relationships. We believe that our findings provide valuable insights on the effectiveness of existing dialog disentanglement approaches and these findings would promote a better application of dialog disentanglement in software engineering.

==> Sections/0-todo.tex <==
%1. metrics? measure?
%2. check IJCAI-empirical: threat and validity
% 3. reference format, balance
%4. figure 1 add a, b
% 5. check all the numbers, make sure they are correct and well-formatted.
% 6. Migration, migrat* ->Original
% 7. incomplete incorrect 
% 8. four model update
% 9. mixing up topics
% 10. format numbers under 10
% 11. check ref, format, caption
% 12. add dataset url
% 13. split Figure 2 

Celia:
% 2. Can we be consistent? software-related chat, yes software-related messages, no software-related dialogues? yes

% We use italic for DLD, PtrNet,..., so be consistent

% check abstract online

% check grammar problems https://www.grammarly.com/

% fix Section 5 figures

submit

carefully reading 3+ times

% improve Fig 1

submit 


==> Sections/experiment_result/RQs.tex <==
\section{Experiment and Result}\label{section4}

In this section, we compare and select the best performance model on software-related chat. We also introduce the most appropriate metric to measure human satisfaction: the DLD, and filter the bad cases with human annotation and card sorting.
% Significance analysis and hypothesis testing are used to best model selection on POG dataset. Disentanglement quality assessment and error analysis are incorporated in metrics reconciliation. Bad cases classification and card analysis are involved in incorrect disentanglement analysis.

% \subsection{Research Questions}
% \begin{itemize}
% \item RQ1 (Model Comparison): Which baseline approach is the best according to existing measurement? 
% \item RQ2: Are existing measurement in accordance with human judgement?
% \item RQ3: What mistakes did the SOTA model make in developer dialogues?
% \end{itemize}


==> Sections/introduction.tex <==
\section{Introduction}
% The {\it IJCAI--21 Proceedings} will. If your paper is accepted, please carefully read the notifications you receive, and check the proceedings submission information website\footnote{\url{https://proceedings.ijcai.org/info}} to know how many pages you can finally use. That website holds the most up-to-date information regarding paper length limits at all times. Please notice that if your track allows for a special references-only page, the {\bf references-only page(s) cannot contain anything else than references} (i.e.: do not write your acknowledgments on that page or you will be charged for it).

% \begin{figure}[htbp]
% \centerline{\includegraphics[scale=0.35]{Diagram/Annotation_GT.pdf}}
% \caption{Dialog disentanglement and error analysis. Different text color indicates G-T dialogue clusters, and color grey shows the missing sentence. The brown connecting denotes the automatic disentangled dialogues. Because of the semantic similarity, {\it Line 5} and {\it Line 6} are disentangled into same cluster.\lin{I think we can remove this for spacing}}
% \label{disentanglement_concept}
% \end{figure}

% With the development of Open-Source Project, discussions around these projects have grown enormously. Developers of projects can refer to chat messages to gather information of issues, feature requests, bug reports and Q\&A messages {\it et al.}. Traditionally, researchers have chosen wide-used platforms to acquire datasets. StackOverflow\footnote{\url{https://www.stackoverflow.com}} is a Q\&A platform for developers to consult the solution of encountered bugs; Github\footnote{\url{https://www.github.com/}} has issues for project maintenance. In the research field of software engineering, Moran~\shortcite{esecfse15bugs} enhances the quality of Android APP bug reporting with tracing Github issues; Shi {\it et al.}~\shortcite{ase17fra} leverage Github dataset for mining the linguistic pattern of feature requests; Stefanie {\it et al.}~\shortcite{ese20dialogue} analyse the Q\&A flows within StackOverflow dataset.

% However, the existing platforms are limited in real-time information, and existing datasets are not strictly categorized by open source projects. Therefore, the real-time chat rooms are applied for enhancing the data quality. Gitter\footnote{\url{https://www.gitter.im/}} and Slack\footnote{\url{https://www.slack.com/}} are real-time chat rooms for communications between developers and programmers. Because these platforms contain massive natural language discussions, the noise and mixture of dialogues are widespread in raw data. Dialogue disentanglement, aiming to search the reply relationship in complex conversations, is the strategy to untangle the mixed utterances and extract information. Chatterjee~\shortcite{disentangleanalysis2,disentangleanalysis3} conducts empirical researches on models application on Slack chats; Shi {\it et al.}~\shortcite{icse20fra} detects the hidden feature requests from Github issues with disentangled Slack chats. The reliability of disentanglement strongly affect the accuracy of further software engineering tasks.

% In order to elaborating the availability of existing disentanglement models, we propose several systematic research steps for our empirical study. We 1) first collect natural-language chat messages from Gitter website and build the project-based dataset with user engagement based filtering and two steps tradeoffs. Then, we 2) perform two training strategies ({\bf Migration} and {\bf Retraining}) to select the best model on our dataset. The BiLSTM~\cite{bilstm2017usage,ijcai20e2e}, BERT~\cite{bertbase,li2020dialbert,ijcai20e2e}, E2E~\cite{ijcai20e2e} and FF~\cite{acl19disentangle} are investigated, in order to evaluating the effectiveness of baselines and deciding the SOTA model.

% With the comparison between different metrics with SOTA prediction, we find that even the weakness of SOTA baseline is nonnegligible. We 3) rate the $<P_D,T_D>$ pairs with human annotation, and introduce {\it Dialogue-Levenshtein Distance} (DLD)~\cite{levendist,levendist2} for better fitting the rates. Finally, we 4) filter the incorrect disentangled dialogues according to human satisfaction, and elicit knowledge with card sorting~\cite{cardsorting1,cardsorting2}. The taxonomy of bad cases also provide directions for further model optimization.


% Our main contributions are shown as follows:
% \begin{itemize}
%     \item We propose the first project-based dataset with platform Gitter. The convinced dataset is established, which is suitable for software engineering tasks.
%     \item We select the SOTA model with performance on our dataset. A more practical metric DLD is chosen for analyzing bad cases.
%     \item We conduct a card sorting on filtered on incorrect dialogues with DLD threshold. Results provide more practical optimization for improving model generalization.
% \end{itemize}\footnote{\url{https://www.slack.com/}}\footnote{\url{https://www.freenode.net/}}



% Recent studies indicate that the usage of online chatting is gaining popularity and plays a significant role in {\it Software Engineering} (SE) tasks. Developers are turning into these public live chat platforms, such as Slack, Gitter\footnote{\url{https://www.gitter.im/}} and Freenode, for searching defect resolution and sharing opinions and interesting insights.
% Online chatting messages have the advantages of real-time and text rich, which usually incorporate the existing problems and optimization directions of various software projects. 
% Massive online chatting contains valuable information like the intention of live chat usages~\cite{intention_chat}, the hidden feature requests~\cite{icse20fra} and different Q\&A flows~\cite{ese20dialogue} {\it etc.}, which has been widely applied by SE researchers.



% Dialogue disentanglement, which is the strategy of untangling the mixed utterances, is an essential prerequisite for in-depth analysis for analyzing these information. 
% Utterances within the same disentangled dialogue are discussing the same topic, and participants follow a ``reply-to" relationship. 
% Different dialogues are independent, following the characteristics of clustering: ``high cohesion" and ``low coupling". 
% Recently, algorithms and models of disentanglement are progressively proposed by researchers. 
% 
Increasingly, software developers are leveraging live chat platforms such as Gitter and Slack to collaborate, communicate, and coordinate their efforts, especially for the teams that are geographically distributed. 
The conversations on live chat contain a large volume of valuable information for improving software maintenance, including shared knowledge, identified issues, future enhancements, and best practices.
Due the nature of live chat, all the messages appear synchronously. These entangled messages mix all topics together without indication of separate conversations. 
Only when the conversations are disentangled, could in-depth analysis and utilization for those valuable information be performed.

A number of dialogue disentanglement approaches have been proposed in the literature to address the above problem. Early works use handcrafted features for training simple classifiers to analyze the coherence of message-pairs~\cite{disentangle1}. Neural network are then applied to obtain the relationships with the development of deep learning, such as FeedForward (FF)~\cite{acl19disentangle}, CNN~\cite{jiangdisentangle} and BiLSTM~\cite{bilstm2017usage} {\it etc.}. Sequential context based models are introduced with pre-trained BERT~\cite{li2020dialbert} and encoder/decoder technologies~\cite{ijcai20e2e}. To evaluate their approaches , most existing studies use Twitter or Reddit dataset that engaging generally social conversations, such as movies and news. Only Kummerfeld's work evaluate on Ubuntu technical chat but only in a single-project scope.

However, it remains unclear how far we are from effective dialogue disentanglement towards professional and technical software-related chat. First, there is a lack of thorough comparisons of the state-of-the-art dialogue disentanglement approaches on software-related chat. Second, none of previous studies investigate how well existing disentanglement measures reflect human satisfaction. Last but not least, there is a limited understanding of why existing approaches fail to disentangle software-related chat, which can insight future improvement on dialogue disentanglement.

In this paper, we try to fulfill the above insufficiency via an exploratory study on \num{7226} real-world developers' utterances taken from eight popular open source projects. 
First, we compare four baseline dialogue disentanglement approaches according to two training strategies: direct migration across domains and retraining on software-related dialogues. Second, we further investigate how well do existing disentanglement measures reflect human satisfaction. The results show that existing measures cannot correctly indicate the human satisfaction on disentanglement results. 
Therefore, we propose and evaluate a novel measure, named DLD, to complement the existing literature. Third, we summarize four categories of the most frequent appeared bad cases on software-related chat. We believe that the findings and insights we have uncovered will promote a better application of dialog disentanglement in software engineering domain.


% {\it RQ1 (Model comparison): How well do disentanglement models perform on software-related dialogues?}

% {\it RQ2 (Measures for human satisfaction). How well do disentanglement measures reflect human satisfaction?}

% {\it RQ3 (Bad cases analysis) Why does the best disentanglement model fail on software-related dialogues?}

The major contributions of this paper are as follows.
\begin{itemize}
\item We conduct an empirical study on evaluating the baseline disentanglement approaches towards software-related chat. 
\item We propose a novel measure, named DLD, for measuring human satisfaction on disentanglement results.
\item We share a dataset of disentangled software-related dialogs to facilitate the replication of our study and future improvements.
\end{itemize}

%However, disentanglement of online chatting messages is a big challenge, and the existing models have apparent weaknesses when performed on SE tasks. Experiment shows that the disentanglement quality on online chatting dataset is bad, mainly because the existing models consider little about the characteristics of software-related chat. SE dialogues usually have (i) user relationships: the previous close-related users often communicate in the follow-up discussions; (ii) topics: each disentangled dialogue has a simple and concise topic; (iii) entity relationships: the discussed domains have alias and concept relationships with other domains; (iv) interaction patterns: the interaction patterns usually mark the beginning and end of dialogues. For evaluating the effectiveness of existing models on SE dialogues and conclude the bad cases, we conduct the empirical study.

==> Sections/related_work.tex <==
\section{Related Work}
In this section, we summarize the reference works for model analysis in empirical study, and roughly introduce the application of dialogue disentanglement.

\textbf{Evaluation of existing models.}
% Dialogue disentanglement has three basic steps, the first is calculating the similarity between \num{2} different sentences; and then determining the whether these two sentences belong to the same cluster; finally separating the raw data into different dialogues. Elsner and Charniak~\shortcite{disentangle1} first adopt handcrafted method to label features and train classifiers; Shen {\it et al.}~\shortcite{shen-F} choose {\it Weight-SP} to predict message-pair connection. After the widespread of deep learning and neural network, Kummerfeld {\it et al.} propose an {\it IRC} dataset and FF model for predicting the reply between messages; Meheri and Carrenini~\shortcite{bilstm2017usage} choose RNN and BiLSTM for enhancement; Jiang {\it et al.}~\shortcite{jiangdisentangle} propose model CISIR with combination of CNN and a novel similarity ranking. Recently, researchers have paid attention on the pre-trained models and dialog encoder/decoder method. Li {\it et al.}~\shortcite{li2020dialbert} optimize BERT for disentanglement, and Liu {\it et al.}~\shortcite{ijcai20e2e} propose a E2E model with dialogue encoder and session state encoder. These models inspire us for SOTA selection and metrics reconciliation.
Previous works have provided many ideas for conducting this empirical study. The first is baseline comparison with dataset properties: Elsner and Charniak~\shortcite{disentangle1} uses baseline comparisons with one single-project database, and calculates pause length distribution; Mehri and Carenini~\shortcite{bilstm2017usage} conduct the thread length analysis on the same dataset. Then, multi-database research is the basic idea of model migration. Jiang {\it et al.}~\shortcite{jiangdisentangle} experiment the CISIR on three topics' news dataset with ubuntu dataset; Kummerfeld {\it et al.}~\shortcite{acl19disentangle} further request the dataset from other previous researchers to complete the baseline comparison. Finally, the ablation study and retraining method are widely used due to the progress of feature engineering: Li {\it et al.}~\shortcite{li2020dialbert} perform the feature\&future BERT comparison on \num{6} metrics; Liu {\it et al.}~\shortcite{ijcai20e2e} propose the TSL\&DS study and retrain E2E on traditional and new datasets. These methods inspire us to refine our datasets and experiments

\textbf{Application of dialogue disentanglement.}
Since dialogue disentanglement is a emerging technology, researchers have applied it within various tasks. Considering software engineering tasks, Delobelle and BerendtWang~\shortcite{emojidialogue} uses disentanglement to study the Emoji in casual conversations. Wang {\it et al.}~\shortcite{slack_enteprises} analyze the employees collaborate; Shi {\it et al.}~\shortcite{icse20fra} extract feature requests with disentangled dialogues. Since the application of disentanglement with online chatting and software engineering is quite few, our empirical study is valuable for follow-up researchers.
% \lin{This paper seems the most related, what's the difference with ours}

% As for the Q\&A mining, Liu {\it et al.}~\shortcite{kdd19conv} tag the candidate dialogues with \num{51} key points and propose a {\it Leader-Writer} network to summarize the dialogues; Qu {\it et al.}~\shortcite{userintent19} classify the {\it MSDialog} into \num{12} labels for preprocessing. The above papers provide ideas for our card sorting.\lin{I don't think this is quite related}
